The Square Sieve and a Lang-Trotter Question for Generic Abelian Varieties

Let $A$ be a $g$-dimensional abelian variety over $\mathbb{Q}$ whose adelic Galois representation has open image in $\text{GSp}_{2g} \widehat{\mathbb{Z}}$. We investigate the endomorphism algebras $\text{End}(A_p) \otimes \mathbb{Q} = \mathbb{Q}( \pi_p )$ of the reduction of $A$ modulo primes $p$ at which this reduction is ordinary and simple. We obtain conditional and unconditional asymptotic upper bounds on the number of primes at which this "Frobenius field" is a specified number field and, when $A$ is two-dimensional, at which the Frobenius field contains a specified real quadratic number field. These investigations continue the investigations of variants of the Lang-Trotter Conjectures on elliptic curves.

==> BibFiles/BibTemplates.tex <==
%%%  see https://verbosus.com/bibtex-style-examples.html  %%%

%%% use note = {} to include the LABEL in the bibliography, to get a useful reference page 
%%% comment out "\AtEveryBibitem{\clearfield{note}}" on CustomCommands.tex to get back to a usual bibliography

@article{,
note = {},
journal = {},
number = {},
pages = {},
title = {},
author = {},
volume = {},
year = {},
}
%%%%%%%%%%%%%%%%%%%%%
@book{,
note = {},
author = {}, 
title  = {},
publisher = {},
year      = {},
volume    = {},
series    = {},
edition   = {},
}
%%%%%%%%%%%%%%%%%%%%%%
@phdthesis{,
note = {},
author = {}, 
title = {},
school = {},
year = {},
}
%%%%%%%%%%%%%%%%%%
@proceedings{,
note = {},
title = {},
year = {},
editor = {},
volume = {},
series = {},
organization = {},
publisher = {},
}
%%%%%%%%%%%%%%%%5
@incollection{ ,
author = {},
title = {},
editor = {},
booktitle = {},
publisher = {},
address = {},
year = {},
pages = {}
}
